Spectral Lower Bounds on the I/O Complexity of Computation Graphs

We consider the problem of finding lower bounds on the I/O complexity of arbitrary computations in a two level memory hierarchy. Executions of complex computations can be formalized as an evaluation order over the underlying computation graph. However, prior methods for finding I/O lower bounds leverage the graph structures for specific problems (e.g matrix multiplication) which cannot be applied to arbitrary graphs. In this paper, we first present a novel method to bound the I/O of any computation graph using the first few eigenvalues of the graph's Laplacian. We further extend this bound to the parallel setting. This spectral bound is not only efficiently computable by power iteration, but can also be computed in closed form for graphs with known spectra. We apply our spectral method to compute closed-form analytical bounds on two computation graphs (the Bellman-Held-Karp algorithm for the traveling salesman problem and the Fast Fourier Transform), as well as provide a probabilistic bound for random Erdos Renyi graphs. We empirically validate our bound on four computation graphs, and find that our method provides tighter bounds than current empirical methods and behaves similarly to previously published I/O bounds.

==> extras/normalized_laplacian.tex <==
We further define the normalized Laplacian $\mathcal{L} = D^{-1/2}LD^{-1/2}$. The normalized Laplacian is often useful because the spectra are generally more even than the regular laplacian. We can define an analagous result to Equation \ref{laplacianedges}. For $S \subseteq V$, define the volume of $S$ as: $vol(S) = \sum_{v \in S} d(v).$
Then with $x$ as a one-hot encoding of $S$, define $y = D^{1/2}x = x_i \sqrt{d(v_i)}$. Then $||y||_2^2 = x^T D x = vol(S)$. Letting $\hat{y}$ be the unit vector $\frac{y}{||y||_2}$, we have:
\begin{equation}
    \hat{y}^T \mathcal{L}_G \hat{y} = \frac{x_i^T L x_i}{||y||_2^2} = \frac{1}{vol(S)} \sum_{(u,v) \in \partial S} w(u,v)
\end{equation}

% ------
We can relax this bound slightly in order to frame the problem in terms of the normalized Laplacian. Define $Y = \tilde{D}^{1/2}X\hat{W}^{(k)}\tilde{D}_p^{-1/2}$, where $\tilde{D} \in \mathbb{R}^{n \times n}$ is the degree matrix of $\tilde{G}$ and $\tilde{D}_p \in \mathbb{R}^{k \times k}$ is a diagonal matrix where the ith diagonal entry is the volume of the ith segment: $(\tilde{D}_p)_{ii} = vol(P^{(X,k)}_i)$. Note then that the columns of $Y$ have norm 1 and are orthogonal to each other, so $Y^TY = I$. 


Let $vol(S^*) = \inf_{S \in P_k} vol(S)$. Notably, based on our weighting of $\tilde{G}$, we can lower bound the volume of any one of our partition as:
$$vol(S^*) \geq (\lfloor n/k\rfloor)(1+ \frac{\min_v d_{in}(v)}{\max_v d_{out} (v)}).$$

Then we can write:
\begin{align*}
    \sum_{S \in P_k} \sum_{(u,v) \in \partial S} \frac{1}{d_{out}(u)} &\geq vol(S^*) \sum_{S \in P_k} \frac{1}{vol(S)}\sum_{(u,v) \in \partial S} \frac{1}{d_{out}(u)}\\
    &= vol(S^*) tr(\tilde{D}_p^{-1/2} \hat{W}^{(k)^T} X^T \tilde{D}^{1/2} \mathcal{L} \tilde{D}^{1/2} X \hat{W}^{(k)}\tilde{D}_p^{-1/2})\\
    &= vol(S^*) \tr(Y^T \mathcal{L} Y)\\
    &\geq (\lfloor n/k\rfloor)(1+ \frac{\min_v d_{in}(v)}{\max_v d_{out} (v)}) \tr(Y^T \mathcal{L} Y)
\end{align*}

After relaxing the constraints on $Y$ so that $Y^TY = I$ and removing our , we get that the following problem is a lower bound on our objective (\textbf{OPT 4}). 

\begin{align*}
    \text{minimize}_X \quad & \sup_{k} (\lfloor n/k\rfloor)(1+ \frac{\min_v d_{in}(v)}{\max_v d_{out} (v)}) \tr(Y^T \mathcal{L}Y) - 2 k M\\
    & Y^TY = I
\end{align*}
% -------

We note that the above bound leverages the spectra of the Laplacian. If the spectra have high variance, then the bound deteriorates. It is thus advantageous to state a version of this bound that uses the normalized Laplacian $\mathcal{L}$, because the spectra of the normalized Laplacian often tend to be more even. 
\begin{theorem}[Normalized Laplacian Eigenvalue Bound]\label{normlapbound}
\begin{equation} J^* \geq \sup_k (\lfloor n/k\rfloor)(1+ \frac{\min_v d_{in}(v)}{\max_v d_{out} (v)}) \sum_{i=1}^k \lambda_i(\mathcal{L}) - 2 k M \end{equation}

\end{theorem}

\begin{proof}
We begin by solving \textbf{OPT 4}. Firstly, we note that since $Y^TY = I$, and $Y$ is rank $k$, $YY^T$ has an eigenvalue $1$ of multiplicity $k$ (with eigenvectors as the columns of $Y$) and eigenvalue 0 with multiplicity $n-k$. By \cite{finke1987quadratic} we note that for symmetric $AB$, $tr(AB) \geq \langle \lambda, \mu \rangle_-$. Therefore for any $Y$ such that $Y^TY = I$ we have that
$tr(Y^T \mathcal{L} Y) = \tr(\mathcal{L} Y Y^T) \geq \sum_{i=1}^k \lambda_i(\mathcal{L}).$
In total then we get the bound:
\begin{equation*} 
J^* \geq \sup_k (\lfloor n/k\rfloor)(1+ \frac{\min_v d_{in}(v)}{\max_v d_{out} (v)}) \sum_{i=1}^k \lambda_i(\mathcal{L}) - 2 k M 
\end{equation*}
completing the proof.
\end{proof}




==> sections/tightened_eig.tex <==
While the bound in Theorem \ref{laplacianbound} is easy to analyze when given closed form solutions of the computation graph, we can actually improve our bounds by taking a closer look at the role of the inputs in our partitions. We first prove the following theorem:

\begin{theorem}
Let $\tilde{G}$ be the transformed weighted, undirected graph of $G$ as specified in Section TODO. Let $\hat{D} \in \mathbb{R}^{n - |V_{in}| \times n - |V_{in}|}$ be a diagonal matrix of the degrees of $\textit{non-input}$ vertices in $\tilde{G}$. Furthermore, let $\hat{A}$ be the undirected adjacency matrix of the subgraph of $\tilde{G}$ induced by $V/V_{in}$. Let $\hat{L} = \hat{D} - \hat{A}$. 
Then:
$$J^*_G \geq  \inf_{\substack{X \in \mathbb{R}^{n - |V_{in}| \times n - |V_{in}|},\\ X^TX = I}} \sup_{k} \tr(X^T \hat{L} X W^{(k)}) - 2kM$$
\end{theorem}
\begin{proof}

    Let $X$ be some evaluation order on $G$. Suppose then we create an even k-segmentation of the vertices $V$ according to $X$ as in section TODO. Let $u$ be an input vertex, and let $S$ be the partition that $u$ belongs to.

    We note that the ``computation'' of $u$ is simply the first time the input $u$ was read from disk. Since $u$ begins on disk, computing $u$ in $S$ is equivalent to pretending $u$ was ``computed''  outside $S$ and then simply loading $u$ from either disk or cache during the computation of $S$ as we would load any other parent of a vertex in $S$ that was computed outside of $S$. We can thus move $u$ out of $S$ into its own partition. We can perform the same manuever for each of the input vertices, creating a new partition $S_{in}$ that contains the input vertices.



    % Rather than treating $V_{in}$ as an operation that needs to be computed in $X$, we instead treat $V_{in}$ as already computed (and on disk). We note that every input has to be read in at least once. 

\end{proof}
